Beyond Local Nash Equilibria for Adversarial Networks

Save for some special cases, current training methods for Generative Adversarial Networks (GANs) are at best guaranteed to converge to a `local Nash equilibrium` (LNE). Such LNEs, however, can be arbitrarily far from an actual Nash equilibrium (NE), which implies that there are no guarantees on the quality of the found generator or classifier. This paper proposes to model GANs explicitly as finite games in mixed strategies, thereby ensuring that every LNE is an NE. With this formulation, we propose a solution method that is proven to monotonically converge to a resource-bounded Nash equilibrium (RB-NE): by increasing computational resources we can find better solutions. We empirically demonstrate that our method is less prone to typical GAN problems such as mode collapse, and produces solutions that are less exploitable than those produced by GANs and MGANs, and closely resemble theoretical predictions about NEs.

==> fig1b/fig_unifake_convergence_vert.tex <==
{
\newlength{\mywOneB}
\setlength{\mywOneB}{0.89\columnwidth}
\begin{figure}[tb]
\centering
\scalebox{0.7}{
\begin{tabular}{cc}
% we need these plots - no need for more samples - these DO NEED CROPPING
% /attempt3/prog_MOG_2017-09-10_012502-GANrand9".png
% /attempt3/prog_MOG_2017-09-11_000831-scr7unifakev1_random9_GAN_eqLRs".png
    \hspace{-4mm}
\subfloat{\includegraphics[width = \mywOneB]{fig1b_1.png}} \\
\subfloat{\includegraphics[width = \mywOneB]{fig1b_2.png}} 
\end{tabular}
}
\caption{Convergence without (top) and with (bottom) adding uniform fake data.
    Shown is the payoff as a function of the number of iterations of PNM. 
    Tests that do not yield positive payoff (red line $< 0$) are not 
    added to the mixture.
}
\label{fig:unifakeconv}
\end{figure}
}


==> figs-exploit_variance/exploit_variance.tex <==

\begin{figure*}[p]
\centering
\begin{tabular}{ccc}


\subfloat{\includegraphics[trim={1cm 0.5cm 0.5cm 1cm},clip, scale = 0.4]{gan_gen_br1.png}} &
\subfloat{\includegraphics[trim={1cm 0.5cm 0.5cm 1cm},clip, scale = 0.4]{gan_gen_br2.png}} &
\subfloat{\includegraphics[trim={1cm 0.5cm 0.5cm 1cm},clip, scale = 0.4]{gan_gen_br3.png}} \\


% PNM 16

\subfloat{\includegraphics[trim={1cm 0.5cm 0.5cm 1cm},clip, scale = 0.4]{pnm_gen_br1.png}} &
\subfloat{\includegraphics[trim={1cm 0.5cm 0.5cm 1cm},clip, scale = 0.4]{pnm_gen_br2.png}} &
\subfloat{\includegraphics[trim={1cm 0.5cm 0.5cm 1cm},clip, scale = 0.4]{pnm_gen_br3.png}}\\


\end{tabular}

\caption{CAPTION}
\label{fig:newresults}
\end{figure*}



         
%\end{document}

